Toward Neural-Network-Guided Program Synthesis and Verification

We propose a novel framework of program and invariant synthesis called neural network-guided synthesis. We first show that, by suitably designing and training neural networks, we can extract logical formulas over integers from the weights and biases of the trained neural networks. Based on the idea, we have implemented a tool to synthesize formulas from positive/negative examples and implication constraints, and obtained promising experimental results. We also discuss two applications of our synthesis method. One is the use of our tool for qualifier discovery in the framework of ICE-learning-based CHC solving, which can in turn be applied to program verification and inductive invariant synthesis. Another application is to a new program development framework called oracle-based programming, which is a neural-network-guided variation of Solar-Lezama's program synthesis by sketching.

==> app-sec4.tex <==
\section{Additional Information for Section~\ref{sec:rel}}
\label{app:sec4}

\subsection{On CLN2Inv vs Our Approach for Code2Inv Benchmark}

Ryan et al.~\cite{DBLP:conf/iclr/RyanWYGJ20} reported that
CLN2Inv (\url{https://github.com/gryan11/cln2inv}) could solve all the 124 problems
of the Code2Inv Benchmark set. As far as we checked, however, their tool has the following
limitation.
First, the shape of invariants that can be learned is restricted, and tailor-made
for finding invariants for programs consisting of a single loop. More specifically,
they conjoin formulas found by CLN with the constraints on variable bounds (of the form \(x \diamond c\),
with \(\diamond\in\set{\le, \ge}\)) gathered by sample data and constant files.
Second, probably as a consequence of the first limitation,
for the problems \(\#1, \#2, \#94\), the tool actually fails to find linear invariants
(we confirmed this by removing the samples for \(x^2, xy, y^2\) from, e.g.
\url{https://github.com/gryan11/cln2inv/blob/master/benchmarks/code2inv/csv/1.csv}
and running the tool). We have also inspected an implementation of G-CLN~\cite{DBLP:conf/pldi/YaoRWJG20},
 available at \url{https://github.com/jyao15/G-CLN};
as far as the Code2Inv benchmark is concerned, it seems to have similar limitations.

In contrast, our combination of \hoice{} and \NNG{} can solve all the 124 problems (actually,
all but one can be solved by plain \hoice{}), given only CHC problems as inputs;
the C source code, sample files, and constant files are not required.


\subsection{On SVM vs NN}
Figure~\ref{fig:svm} shows the qualitative difference between the classifications
by SVM vs NN.
 Small circles denote positive examples,
    and the white space is filled with negative examples.
    The dashed line shows a linear classifier typically
    output by a SVM, while the thick line shows the (complete) classifier output by
    a NN.
    
\begin{figure}[h]
  \begin{center}
    \includegraphics[scale=0.4]{SVMvsNN}
    \vspace*{-.3cm}
    \end{center}
  \caption{SVM vs NN.}
    \label{fig:svm}
\end{figure}



==> exp.tex <==
\section{Experiments}

\subsection{Learning from Positive/Negative Samples}

\nk{Experiments on classifications of two-dimensional data (gathered from
  the experiments in the directory \texttt{2d-nobias});
  comparison on vairous designs of NNs, such as activation functions,
the number of hidden nodes, the number of layers, ...}

\subsection{Ice Learning}

\nk{Experiments on learning in the presence of implication constraints (gathered from
the experiments in the directory \texttt{chc})}



==> pre.tex <==
\section{Preliminaries}
\nk{Probably we do not need this section. It would be sufficient to
  explain the four-layer NNs in Section 3.1.}
\begin{itemize}
\item
  Basics on neural networks
\item
  Basics on program synthesis/verification? (sketching, ICE-based learning, ...)
\end{itemize}

